RecInDial: A Unified Framework for Conversational Recommendation with Pretrained Language Models

Conversational Recommender System (CRS), which aims to recommend high-quality items to users through interactive conversations, has gained great research interest recently. A CRS is usually composed of a recommendation module and a generation module. In the previous work, these two modules are loosely connected in the model training and are shallowly integrated during inference, where a simple switching or copy mechanism is adopted to incorporate recommended items into generated responses. Moreover, the current end-to-end neural models trained on small crowd-sourcing datasets (e.g., 10K dialogs in the ReDial dataset) tend to overfit and have poor chit-chat ability. In this work, we propose a novel unified framework that integrates recommendation into the dialog (RecInDial) generation by introducing a vocabulary pointer. To tackle the low-resource issue in CRS, we finetune the large-scale pretrained language models to generate fluent and diverse responses, and introduce a knowledge-aware bias learned from an entity-oriented knowledge graph to enhance the recommendation performance. Furthermore, we propose to evaluate the CRS models in an end-to-end manner, which can reflect the overall performance of the entire system rather than the performance of individual modules, compared to the separate evaluations of the two modules used in previous work. Experiments on the benchmark dataset ReDial show our RecInDial model significantly surpasses the state-of-the-art methods. More extensive analyses show the effectiveness of our model.

==> sections/Limitations.tex <==
\section{Limitations}
In this section, we mainly talk about the limitation of single-reference evaluation problem in an open-ended conversation recommendation system and the limitation of our model when handling new items. 
\paragraph{The Limitation of Single-Reference Evaluation}. As you can see in Table \ref{tab:intro_case} or Table \ref{fig:case}, there is only one ground truth movie item for every utterance. Under such a setting, humans may even not suggest the item that is the same as the ground truth. Therefore, it may result in the Recall@K (K = 1, 10, 50) could not reflect the true performance of a system well. Besides, the sizes of the currently available datasets are quite small which exacerbates the impact of the single-reference evaluation.
\paragraph{The Limitation of Handling New Items.} Our framework cannot handle items that are not existed in the training set, since we extend the vocabulary with static item set. However, handling new items that never appear during training is important when applying in a real-world application system. We might resolve it by making the item set dynamic. We leave it to our future work. 


==> tables/finetune_different_layers.tex <==
\begin{table}[ht]\setlength{\tabcolsep}{0.45mm}\footnotesize
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
\scalebox{0.9}{
\begin{tabular}{lcccccc}
\hline
\multirow{2}{*}{Finetune Layers} & \multicolumn{3}{c}{ \tabincell{c}{{Recall@1}} } & \multicolumn{3}{c}{ \tabincell{c}{{Dist-2}}}
\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
& Att  & MLP & Att+MLP & Att &MLP &Att+MLP \\
\hline
\textsc{0} &1.0 &1.4 &1.6 &31.9 &27.9 &41.2 \\
\textsc{11} &1.3 &0.9 &1.6 &32.9 &42.6 &69.8 \\
\textsc{0,11} &1.2 &1.0 &1.0 &39.5 &32.9 &27.8 \\
\textsc{0,1,10,11} &0.7 &1.0 &1.1 &21.7 &35.5 &31.1 \\
\textsc{all} &0.7 &1.2 & &21.7 &34.5 & \\



\hline
\end{tabular}
}
\end{center}
\vskip -1em
\caption{\label{tab:} 
Main comparison results on recommendation. R@k refers to Recall@k (k=1, 10 and 50). 
}
\vskip -0.5em
\end{table}

==> tables/human_eval_scoring.tex <==
\begin{table}[ht] 

\begin{center}
\scalebox{0.9}{
\begin{tabular}{l|p{7.2cm}}
\hline 

Score & Fluency \\
\hline
\multirow{2}{*}{0} &The response has many grammar mistakes. \\
 & The response is hard to understand.\\
 \hline
\multirow{2}{*}{1} & The response has minor grammar mistakes.  \\
& Some part of the response is hard to understand. \\
\hline
2& The response is in correct grammar and easy to understand. \\
\hline
% \hline

\end{tabular}
}
\end{center}





\begin{center}
\scalebox{0.9}{
\begin{tabular}{l|p{7.2cm}}
\hline 
% \multicolumn{2}{c}{}  \\
% \hline
Score & Coherence \\
\hline
\multirow{4}{*}{0} &  The response is not related with the context.  \\
 & The response simply repeats the context. \\
 & The response has obvious conflicts with the context. \\
 \hline
\multirow{2}{*}{1} & The response has minor conflicts with the context. \\
& There are some minor logic conflicts in the response. \\
\hline
2& The response is coherent with the context. \\
\hline
% \hline

\end{tabular}
}
\end{center}

\begin{center}
\scalebox{0.9}{
\begin{tabular}{l|p{7.2cm}}
% \hline 
% \multicolumn{2}{c}{}  \\
\hline
Score & Informativeness \\
\hline
\multirow{4}{*}{0} & The response does not contain any information.  \\
 & This response just repeats the context and fails to bring any additional information.
\\
 & The information is invalid, as the coherence score is 0. \\
 \hline
\multirow{2}{*}{1} & The information has conflicts with common sense. \\
& There are factual errors in the response. \\
\hline
2& The response contains appropriate and correct information. \\
\hline
% \hline

\end{tabular}
}
\end{center}

\vskip -1em
\caption{\label{tab:human_eval_scoring} Scoring details for human evaluation. 
}
\vskip -1.5em
\end{table}

==> tables/table_example.tex <==
\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:example}
\end{table}
